Measurement of Spin Correlations in $t\bar{t}$ Events from $pp$ Collisions at $\sqrt{s}$ = 7 TeV in the Lepton + Jets Final State with the ATLAS Detector

The top quark decays before it hadronises. Before its spin state can be changed in a process of strong interaction, it is directly transferred to the top quark decay products. The top quark spin can be deduced by studying angular distributions of the decay products. The Standard Model predicts the top/anti-top quark ($t\bar{t}$) pairs to have correlated spins. The degree is sensitive to the spin and the production mechanisms of the top quark. Measuring the spin correlation allows to test the predictions. New physics effects can be reflected in deviations from the prediction. In this thesis the spin correlation of $t\bar{t}$ pairs, produced at a centre-of-mass energy of $\sqrt{s} = 7\,$TeV and reconstructed with the ATLAS detector, is measured. The dataset corresponds to an integrated luminosity of $4.6~\text{fb}^{-1}$. $t\bar{t}$ pairs are reconstructed in the $\ell$+jets channel using a kinematic likelihood fit offering the identification of light up- and down-type quarks from the $t \rightarrow bW \rightarrow bq\bar{q}'$ decay. The spin correlation is measured via the distribution of the azimuthal angle $\Delta\phi$ between two top quark spin analyzers in the laboratory frame. It is expressed as the degree of $t\bar{t}$ spin correlation predicted by the Standard Model, $f_{\text{SM}}$. The results of \begin{align*} &f_{\text{SM}}( \Delta\phi(\text{charged lepton, down-type quark} )) &= 1.53 \pm 0.14\,\text{(stat.)} \pm 0.32\,\text{(syst.)}, \\ &f_{\text{SM}} ( \Delta\phi(\text{charged lepton, b-quark} )) &= 0.53 \pm 0.18\,\text{(stat.)} \pm 0.49\,\text{(syst.)}, \\ &f_{\text{SM}} ( \Delta\phi(\text{combined})) &= 1.12 \pm 0.11\,\text{(stat.)} \pm 0.22\,\text{(syst.)}, \end{align*} are consistent with the Standard Model prediction of $f_{\text{SM}}= 1.0$.

==> appendices/lepflavcons.tex <==
\section{Consistency of Results Across Lepton Flavours}
\label{sec:app_lepflavcons}


For consistency across different lepton flavours a further set of plots is provided.  For each analyser, jet and b-tag multiplicity bin, the SM prediction of \dphi\ is plotted for the \ejet\ (red lines) and the \mujet\ (blue lines) channel as well as the according data. Ratios of data (solid) to prediction (dashed) are also shown as well as the ratio of these two ratios (green). These plots are provided for the \dQ\ in Figure \ref{fig:lepflavorcons_dQ} and the for \bQ\ in Figure \ref{fig:lepflavcons_bQ}.

\begin{figure}[htbp]
\begin{center}
\includegraphics[width=0.45\textwidth]{images/appendix/flavorcomp/4jex_1bex.eps} 
\includegraphics[width=0.45\textwidth]{images/appendix/flavorcomp/4jex_2bin.eps} \\
\includegraphics[width=0.45\textwidth]{images/appendix/flavorcomp/5jin_1bex.eps} 
\includegraphics[width=0.45\textwidth]{images/appendix/flavorcomp/5jin_2bin.eps} 
\end{center}
\caption{The SM prediction (dashed) of $\Delta \phi(l,d)$ for the \ejet\ (red lines) and the \mujet\ (blue lines) channel as well as the according data (solid). Ratios of data to prediction are also shown as well as the ratio of these two ratios (green). 
}
\label{fig:lepflavorcons_dQ}
\end{figure} 

\begin{figure}[htbp]
\begin{center}
\includegraphics[width=0.45\textwidth]{images/appendix/flavorcomp/4jex_1bex_bQ.eps} 
\includegraphics[width=0.45\textwidth]{images/appendix/flavorcomp/4jex_2bin_bQ.eps} \\
\includegraphics[width=0.45\textwidth]{images/appendix/flavorcomp/5jin_1bex_bQ.eps} 
\includegraphics[width=0.45\textwidth]{images/appendix/flavorcomp/5jin_2bin_bQ.eps} 
\end{center}
\caption{The SM prediction (dashed) of $\Delta \phi(l,b)$ for the \ejet\ (red lines) and the \mujet\ (blue lines) channel as well as the according data (solid). Ratios of data to prediction are also shown as well as the ratio of these two ratios (green). 
}
\label{fig:lepflavcons_bQ}
\end{figure} 

